Jupybara: Operationalizing a Design Space for Actionable Data Analysis and Storytelling with LLMs

Mining and conveying actionable insights from complex data is a key challenge of exploratory data analysis (EDA) and storytelling. To address this challenge, we present a design space for actionable EDA and storytelling. Synthesizing theory and expert interviews, we highlight how semantic precision, rhetorical persuasion, and pragmatic relevance underpin effective EDA and storytelling. We also show how this design space subsumes common challenges in actionable EDA and storytelling, such as identifying appropriate analytical strategies and leveraging relevant domain knowledge. Building on the potential of LLMs to generate coherent narratives with commonsense reasoning, we contribute Jupybara, an AI-enabled assistant for actionable EDA and storytelling implemented as a Jupyter Notebook extension. Jupybara employs two strategies -- design-space-aware prompting and multi-agent architectures -- to operationalize our design space. An expert evaluation confirms Jupybara's usability, steerability, explainability, and reparability, as well as the effectiveness of our strategies in operationalizing the design space framework with LLMs.

==> icebox.tex <==
% assess the dimensions' validity and informing tool
%To validate and enrich the design space outlined in Section~\ref{preliminary design space}, w
We conducted formative interviews with nine data analysts. We aimed to understand analysts' workflows, considerations, and challenges in actionable EDA and storytelling, as well as to gauge their attitudes toward AI assistance. In addition, we ran a \add{participatory design exploration} with participants to explore interfaces and interaction techniques in Jupyter Notebook~\cite{kluyver2016jupyter} that would facilitate human-AI collaboration in EDA and storytelling. We focused on Jupyter Notebook because of its popularity among data analysts for EDA. %with recent received much research attention and which we aimed to integrate AI assistance into.

\subsection{Participants} 
We recruited nine participants (\textbf{P1}~-~\textbf{P9}\add{; four men, four women, and one non-binary individual}) with extensive experience in actionable EDA and storytelling \add{from X (formerly Twitter) and three Slack workspaces frequented by data analysts}. Participants represented diverse backgrounds: five were professional data analysts from varying industries, such as environmental science, retail, and education; three were PhD students in natural language processing, human-centered design and engineering (HCDE), and visualization; one was a master's student in HCDE. Participants reported a maximum of 10 years and a minimum of 3 years of experience with data analysis (\textit{mean} = 5.2). \add{We screened participants using an intake survey where they detailed their actionable EDA and storytelling experience, which they later elaborated during interviews. Professional data analysts primarily performed these activities as part of their job, such as drafting environmental policy proposals or creating sales strategies. Graduate students, on the other hand, conducted them for research, e.g., quantitatively comparing human-AI interaction designs and advocating for a specific design in research papers.}

\subsection{Study Procedure}
The study comprised two consecutive sessions. First, we conducted a semi-structured interview lasting around 30 minutes, in which we asked about participants' actionable EDA and storytelling workflows, how they derived and communicated actionable insights, and challenges they often encountered. Toward the end of the interview, we explored how analysts envisioned incorporating AI assistance into EDA and storytelling workflows, including the roles they would like the AI to play and the stages at which they would benefit from AI support.

%The targeted cell design exposes an input area via a popover specific to each cell. The inline cell design places input areas in separate cells between normal notebook cells. The side panel design adds a separate, application-style interface by the side of the main working area of the notebook.

Next, we engaged participants in a 15-minute \add{participatory design exploration} around interaction techniques and interfaces for human-AI collaboration in Jupyter Notebook. Inspired by McNutt~\etal's design space for AI assistants in computational notebooks~\cite{mcnutt2023design}, we initially presented participants with three interfaces for inputting natural language commands: targeted cell, inline cell, and side panel (see Supplemental Materials). We then sought feedback on the suitability of each interface for invoking different types of AI assistance, such as generating responses in EDA and presenting data stories. Finally, we opened a virtual whiteboard and invited participants to sketch alternative designs and articulate their affordances. \add{To encourage deeper discussion, we adopted the perspective of a system user as appropriate, posing questions and scenarios that might arise in their workflows to inspire further designs, thoughts, and discussions, guided by user needs and preferences.}

All sessions took place online. Participants were compensated with a \$20 Amazon gift card. We recorded audio and video for all study sessions. \add{A thematic analysis of the interviews was performed by one of the authors and subsequently refined through discussions with another author. This analysis initially focused on identifying recurring characteristics and challenges in actionable EDA and storytelling workflows. From these findings, we distilled common considerations into a design space, building upon and enriching the framework proposed by Setlur and Birnbaum~\cite{setlur2024can}.} 


\subsection{Findings}
We now summarize the general workflows for actionable EDA and storytelling and some common challenges in the process.

\subsubsection{Workflows for Actionable EDA and Storytelling}
Actionable EDA and storytelling are fluid, integrated, and iterative processes. Its actual workflows vary considerably based on the nature of the dataset, the analyst's domain expertise, initial objectives, and argumentative needs.

\begin{itemize}[leftmargin=0.55cm]
    \item \textbf{Fluidity.} Most participants described their EDA workflows as involving steps such as data cleaning, visualization, transformation, modeling, and hypothesis testing. In data storytelling, they need to organize their findings, verbalize results to highlight actionable insights, and go through revisions. However, these steps are not fixed or linear. As \textbf{P2} noted, ``\textit{There is not a `fixed workflow' for me. The steps I take to analyze a dataset depend on what it has to offer and what my objectives are.}'' Other participants also pointed to factors like ``\textit{surprising findings}'' and ``\textit{guiding analytical questions}'' as influences on the steps they take and the sequence in which they are taken.
    
    \item \textbf{Integration.} In practice, actionable EDA and storytelling are often integrated processes, echoing Gratzl~\etal~\cite{gratzl2016visual}. Especially towards the later stages of projects, analysts often cycle between EDA and storytelling. For example, \textbf{P5} typically ``\textit{switch[es] back and forth between coding and slide-making,}'' citing needs to ``\textit{organize findings in [his] presentation}'' and ``\textit{look for more evidence in the data to support claims in the report.}'' By cycling between EDA and storytelling, analysts can methodically document their findings, continuously refine actionable insights, and effectively plan future analyses.
    
    \item \textbf{Iteration.} Actionable EDA and storytelling workflows are typically messy and iterative, echoing Rule~\etal~\cite{rule2018exploration}. When exploring a dataset, analysts constantly reformulate their hypotheses, mental models, and actionable insights according to the results they observe. \textbf{P8} shrewdly characterized this process as ``\textit{incrementally learn[ing] about the dataset.}'' During EDA, analysts navigate many data facts and cull out interesting ones to further examine. Sometimes, they reach dead-ends and need to revise their approaches; sometimes, analysis paths cross, leading analysts to revisit previous insights and uncover deeper ones.
\end{itemize}


\subsubsection{Challenges in the Workflow} 
\label{challenges}
As intricate and even delicate processes, actionable EDA and storytelling are not without their difficulties. We now dive into four recurring challenges participants brought up.
% These aspects of fluidity, intertwinement, and iteration indicate that actionable EDA and storytelling are intricate and even delicate processes, posing considerable challenges to human analysts as well as to both interaction design and the design of possible AI assistants. We now dive into four recurring challenges participants brought up.

\begin{itemize}[leftmargin=0.55cm]
\item \textbf{C1: Identifying appropriate analytical strategies.} To answer analytical questions, data analysts engage in a series of operations on the data, such as imputation, filtering, and correlation analysis. We refer to a series of concerted analytical operations as an \textit{analytical strategy}. All participants concurred that leveraging appropriate analytical strategies is crucial for extracting valid and compelling insights. Yet, identifying what analytical strategies to use is often challenging, as the process requires statistical expertise, domain knowledge, and familiarity with the dataset. Further, analytical strategies often need to be tailored to specific questions. For instance, \textbf{P8} admitted to often needing to ``\textit{Google around to decide which tests to run.}'' \textbf{P9} highlighted that the seemingly trivial task of handling missing values depends on the nature of the dataset and standard practices in the field. Another curious aspect of how industry know-how affects analytical strategies lies in the choice of adjustments and normalizations. \textbf{P2}, a basketball fan, shared that his analyses of player performance often involved adjusting for playing time and overall team performance. Together, these examples emphasize the difficulty of coordinating multiple dimensions in determining reasonable analytical strategies.

\item \textbf{C2: Tracking insights and analysis history.} Similar to  Weng~\etal~\cite{weng2024insightlens}, we found that tracking insights and analysis history places heavy cognitive burdens on analysts. Every participant agreed that managing insights in EDA is a necessary yet demanding component that pervades the whole EDA and storytelling workflow. \textbf{P1} observed, ``\textit{I pick up findings here and there. It can be challenging to keep track of all of them, considering how many findings I encounter.}'' To document insights, analysts often take notes and screenshots, which provide fodder for insight association and data storytelling. Further, analysts expressed a need to record analysis history, including both the paths that lead to insights and those that result in dead-ends. As \textbf{P9} noted, the fluid and iterative nature of EDA means that the process can be ``\textit{a combination of breadth-first search and depth-first search.}'' Documenting the analytic approaches (i.e., the analytical operations on the data) is not only helpful for informing future analysis and course correction, but also for creating a coherent and persuasive data story. Nonetheless, due to the potentially large number of steps taken to analyze the data, documenting them becomes so time-consuming and mentally taxing that most participants do not engage in this practice systematically, instead relying on memory to recall their analysis paths.

\item \textbf{C3: Finding the right language and narrative structure to effectively convey actionable insights.} 
All participants reported experience in presenting actionable insights in slide decks and written reports. Analysts widely agreed that the language and narrative structure used to verbalize findings significantly impact how the audience perceives them. This is especially true for actionable insights, which inherently carry persuasive intents. Yet, drafting effective actionable data narratives is often a challenging exercise. At the ``lowest'' level, analysts must deliberate word choices when conveying their results. \textbf{P4} observed that ``\textit{there are a million ways you can describe your results, and each has its own meaning.}'' Choosing the right language, then, becomes a matter of ``experience'' and ``gut feeling.'' At a ``higher'' level, analysts need to determine which results to highlight and the appropriate level of detail to provide. These decisions, in turn, depend on a range of factors, such as the prospective actionable insights, the background of the audience, and the context in which the data story is presented, complicating the process of crafting an effective narrative.

\item \textbf{C4: Leveraging relevant domain knowledge to derive actionable insights from data facts.}
Actionable insights do not exist in a vacuum. In order to transform raw data facts from EDA into actionable insights, analysts need to contextualize the results and justify their proposed courses of action by identifying and applying relevant domain knowledge. It can be overwhelming to sift through the vast body of external knowledge required to find the most relevant information. This challenge is particularly pronounced when analysts work across multiple domains or with unfamiliar datasets. According to \textbf{P7}, researching pertinent domain knowledge to augment the narrative is ``\textit{usually harder than getting the results from data analysis.}'' For domains he was unfamiliar with, he often struggled to find relevant sources to augment the narrative. Moreover, even when relevant domain knowledge is identified, analysts need to carefully reason through how to apply it. The particularities in each dataset require analysts to meticulously evaluate how domain knowledge intersects with their data findings. As \textbf{P6} aptly put it, ``\textit{getting results [in EDA] is not the end---it's just the beginning.}''

\end{itemize}
.

\subsection{A Three-Dimensional Design Space}
To map the design space of actionable EDA and storytelling, we asked participants to describe strategies they used to mine and communicate actionable insights and to provide examples. 
The first author, in discussion with the other authors, then coded these strategies. 
We now present this design space in further detail and illustrate how each dimension manifests in both EDA and storytelling. We will also show how our design space subsumes the challenges identified in Section~\ref{challenges} \add{and consider them in the context of relevant literature}.

\subsubsection{\semanticcolor{Semantic Dimension}}
\label{semantic}
The \textcolor{DeepTeal}{semantic dimension} involves precisely specifying the analytical objects (i.e., \textit{what} is being analyzed) and interpreting and tracking the results. It is through language that analysts translate these objects and results into semantic properties they can reason with and about, and convey their nuanced implications with precision to readers. As such, \semanticcolor{semantic precision} precedes and underpins the generation of insights.

\textbf{EDA.} A thorough understanding of the data attributes is essential for any analysis on a dataset. All participants alluded to grasping the semantics of the analytical objects as one of the initial steps in EDA. For instance, analysts often ask themselves: what attributes exist in the dataset? What are their data types? Answering these questions helps analysts develop a clearer sense of \textit{what} is being analyzed and the gamut of analytical questions the dataset can possibly support. To enhance the semantics of a dataset, analysts can further add metadata such as descriptions and data provenance, or join the data with other datasets. 

In addition to defining the semantics of analytical objects, the \textcolor{DeepTeal}{semantic dimension} encompasses ensuring the analytical results carry valid semantics. For instance, in order to glean insights from a visualization, analysts first need to make sure that the visualization is an honest representation of the data, since inappropriate design choices can distort the true patterns in the data and lead to unsound insights downstream. \textbf{P7}'s remark best captures a common approach to this: ``\textit{Every time the code gives me output, I immediately check if the results make sense, and I often catch silly mistakes like using the wrong features in my model.}'' Another critical aspect of the \semanticcolor{semantic dimension} is keeping track of analytical results (echoing \textbf{C2}). Figuratively, analysts construct a ``semantic web'' of results to track and associate data facts, which they grow as they uncover new findings. This ``semantic web'' not only informs subsequent steps in EDA, but also provides raw material for insights, forming a common substrate for both EDA and storytelling.

\textbf{Data Storytelling.} While an accurate \textit{conceptual} understanding of the semantics of analytical objects and results is generally sufficient in EDA, writing a data story further requires analysts to find \textit{proper wordage} to express these semantics, echoing \textbf{C3}. In this sense, data storytelling entails articulating the semantics that are constructed and curated in EDA. When determining the strength of a correlation, for instance, analysts understand that an \textit{r} value of 0.7 indicates a relationship, but they must decide whether to describe the value as ``moderate'' or ``moderately strong.'' (In some circumstances, this issue can be quite fraught: analysts in the US intelligence community, for example, have developed strict guidelines on appropriate numeric ranges for terms such as ``likely.'') Another example is presenting parameter estimates: while a 95\% confidence interval in frequentist terms suggests the range would capture the true parameter in 95\% of repeated studies, a 95\% credible interval in Bayesian analysis indicates a 95\% probability that the true parameter lies within that range. In many cases there are few established guidelines on how to characterize results; analysts must exercise even more caution in choosing the right language. For instance, upon seeing a sharp decline in sales on a line chart, analysts conceptually understand the drop but need to choose the appropriate wording, such as ``fall,'' ``decline,'' or ``crash,'' to precisely convey the extent of the change. Another common strategy for \semanticcolor{semantic precision} is to use domain-specific language. For example, a flat trend in the financial sector might be described as ``steady,'' whereas in weather forecasting, ``unchanged'' would be a more suitable term. 
% In summary, these examples demonstrate the power of language in precisely communicating the nuances of analytical results---and the need to be careful in doing so.


%%%
\add{Our formulation of the \semanticcolor{semantic dimension} also aligns with the literature, which emphasizes the importance of how meaning is assigned to data and how findings from EDA are articulated in a manner that preserves the integrity of the analysis \cite{qiao:2021}. Similar to our findings, prior research suggests that the first step in data storytelling is ensuring that language accurately represents the trends, anomalies, and relationships present in the data~\cite{segel2010narrative,riche2018data}. The semantics behind language also influence how patterns in the data are perceived and understood. Recent work by Bromley and Setlur~\cite{bromley2023difference} reveals how visual features in line charts are associated with different natural language trend descriptors (e.g., ``tanking'' vs. ``decreasing'').  
Thus, \semanticcolor{semantic precision} is essential for accurately conveying insights in a way that is grounded in and congruent with data facts---in sum, truthful.}
%As another example, the term ``anomaly'' suggests a data point deviates significantly from the norm, whereas labeling the point as part of a ``cyclical trend'' implies regular periodicity.
%%%

\subsubsection{\rhetoriccolor{Rhetorical Dimension}}
The \textcolor{RoyalBlue}{rhetorical dimension} involves deploying analytical strategies to derive compelling results and orchestrating the narrative with an eye toward generating, bolstering, and advancing actionable insights. It ensures the trajectory of EDA and the presentation of analytical strategies and results are effectively geared toward persuasively conveying the insights. Hence, the \rhetoriccolor{rhetorical dimension} subsumes the \semanticcolor{semantic dimension} and supports the \pragmaticcolor{pragmatic dimension}.

\textbf{EDA.} Much like rhetorical devices in persuasive writing, analytical strategies in EDA serve vital persuasive purposes. If the semantics of analytical results provide evidence for the insights, then it is through carefully chosen strategies that analysts surface the most relevant findings in EDA (echoing \textbf{C1}). While there could be multiple viable analytical strategies for a given task, there are often nuanced differences in the perspectives they underscore. Consider choosing a dimensionality reduction method: selecting principal component analysis over t-SNE emphasizes the preservation of variance, which could be more effective when arguing for the importance of certain features. When selecting a method for reliable long-term time series forecasting, ARIMA is usually preferred over exponential smoothing for its superior ability to account for trends and seasonality. As another example, choosing between simple correlation and partial correlation can shape how relationships between variables are perceived. Partial correlations, which control for other variables, are particularly useful when arguing for the independent effect of a variable. In addition to deciding which analytical strategies to employ, analysts must document the strategies with which they have experimented during the analytic process (echoing \textbf{C2}). By tracking analytical results (\semanticcolor{semantic dimension}) and strategies (\rhetoriccolor{rhetorical dimension}), analysts can better understand the analytical paths taken, recognize dead ends, expose unexplored questions, and revisit potential blind spots. Insofar as the analytical strategies determine which data facts are revealed and, therefore, which actionable insights are derived, the \rhetoriccolor{rhetorical dimension} critically shapes the direction of EDA. 

\textbf{Data Storytelling.} An effective data story is not merely a compilation of data facts---strategically curated and presented information often resonates more powerfully with the audience (echoing \textbf{C3}). To begin with, analysts must determine which analytical results from EDA to include in the data story, with the aim of identifying a set of data facts that most effectively supports the take-home messages. While it is tempting to include only findings that support the desired narrative, acknowledging contradictory or unexpected results can sometimes enhance the credibility of the story and provide a more balanced perspective. Next, analysts need to decide the order in which to present these findings. A logical and coherent presentation of data facts moves readers ineluctably toward the main conclusions. In this regard, selecting the right connectives with which to convey analytical results is essential for weaving the findings together cohesively. Transitional phrases like ``as a result,'' ``in contrast,'' and ``surprisingly'' elucidate logical connections between data findings and keep the audience engaged. Finally, analysts often need to explicitly narrate the analytical strategies used. Doing so not only clarifies the methodology but also reinforces the validity of the insights. It is also important that the level of detail aligns with the technical background of the audience---tech-savvy readers may appreciate detailed explanations, such as why a regression analysis was chosen, while others might prefer a broader overview. 

Besides structural considerations, thoughtful word choices can also enhance the persuasive power of a data story. For example, while there may exist multiple accurate word choices to describe the same results, each can carry subtly different overtones: in the context of stock prices, ``crash'' and ``fall sharply'' both describe a rapid decline, but the former implies a more severe, potentially irrevocable impact, endowing the word with greater persuasive power to prompt stakeholders to action. To sum up, through structural cohesion and lexical nuance, data stories can better communicate the desired significance and implications of actionable insights.

\add{The \rhetoriccolor{rhetorical dimension} focuses on using \textit{persuasive language }to support specific actions or responses~\cite{perelman:1969}. Effective rhetoric in analytical narratives involves the nuanced usage of language to corroborate actionable insights with clear explanation and communicate the appropriate level of urgency and importance. To lend credibility to insights, analysts often explain how they arrive at data findings~\cite{hullman:2011}. For instance, referencing normalization strategies, which adjust data to account for variations, can underscore the soundness and rigor of the conclusions, as in ``even when adjusted for inflation, consumer prices have shown a consistent increase over the past decade.'' 
Careful word choices can also enhance the argumentative power by conveying the desired degree of significance and nuance. For example, while ``stagnant'' and ``stable'' share similar meanings, they evoke entirely different expectations---``stagnant'' typically carries a negative connotation, suggesting a lack of growth, whereas ``stable'' implies consistency and reliability, which is generally viewed more positively. This kind of \rhetoriccolor{rhetorical} flourish render abstract or complex insights more convincing and engaging to the target audience.}

\subsubsection{\pragmaticcolor{Pragmatic Dimension}}
The \textcolor{BurntSienna}{pragmatic dimension} involves augmenting analytical results with relevant external knowledge to suggest effective courses of action. Building upon precisely conveyed analytical results and carefully chosen analytical strategies, the \pragmaticcolor{pragmatic dimension} culminates in grounded, actionable insights. Whereas the \semanticcolor{semantic} and \rhetoriccolor{rhetorical} dimensions manifest differently in EDA and storytelling, the distinction is much blurrier for the \pragmaticcolor{pragmatic dimension}. Therefore, we address EDA and storytelling together here.

Despite its significance, the concept of insight has been defined in varying ways in the literature. Over time, however, scholars have increasingly moved from viewing insight as mere data facts~\cite{choe2015characterizing} to embracing a more sophisticated perspective that integrates analytical results with domain knowledge~\cite{battle2023we}. This more nuanced view is all the more necessary when discussing actionable insights, since effective decision-making in the wild must contextualize data findings in domain knowledge. In practice, actionable insights can take many forms, such as performance improvement, predictive analysis, and decision support~\cite{schneider2014pragmatics}. \textbf{P3} gave an illustrative example from his consulting services: upon observing stagnation in market growth, particularly among younger demographics, he suggested targeted marketing campaigns on social platforms like TikTok and Instagram. In this case, external knowledge about the influence of popular social media platforms on younger audiences helped him connect data findings to practical solutions. Furthermore, past experiences and domain knowledge must often be adapted to the specific situation. \textbf{P3} recounted another case where his team advised a client to replicate successful marketing campaign strategies from the U.S. in Asian markets, which initially failed to resonate with the Asian audience. Only after accounting for cultural differences and revisiting key assumptions did they see a significant improvement in conversion rates. To give yet another example, while insights presented to senior executives might focus on high-level strategic implications, insights shared with operational teams more likely emphasize implementation details. Although challenging on many fronts, the organic combination of data facts with domain knowledge is essential for generating practical and actionable insights (echoing \textbf{C4}).

\add{The \pragmaticcolor{pragmatic dimension} addresses the \textit{implications and actions} that arise from data analysis, emphasizing the application of the data insights for decision-making~\cite{Kahneman2013,keeney:1992}. This dimension synthesizes various aspects of analyses, such as decision support, predictive analysis, risk management, and resource allocation. In other words, the \pragmaticcolor{pragmatic} aspect is about connecting data to real-world outcomes, i.e., helping frame the insights in terms of potential consequences and suggesting concrete actions. For instance, if a country notices a decline in its Olympic medal count, an analyst can examine historical performance data to identify factors such as changes in training programs, athlete selection processes, or investment in sports facilities that might be impacting performance; each such factor suggests further exploration aimed at identifying possible remediation. By considering the potential actions and practical implications derived from data analysis, the \pragmaticcolor{pragmatic dimension} ensures that insights lead to meaningful and effective outcomes.}




\subsection{Design Considerations for an AI Assistant for Actionable EDA and Storytelling}
Most participants expressed enthusiasm for an AI assistant for actionable EDA and storytelling, citing its ability to automate coding and leverage vast domain knowledge for deeper insights. However, they also raised concerns, such as the risk of hallucination and challenges in verifying the analysis. In order to empower actionable EDA and storytelling with the generative power of LLMs while mitigating associated risks, we distill five design goals from our formative interviews:

\textbf{D1. Integration into analysts' existing EDA and storytelling workflows.} We aim to build a system that respects analysts' existing actionable EDA and storytelling workflows. For easier uptake, our system should build on tools and environments familiar to analysts. Given the tight coupling of EDA and storytelling in communicating actionable insights, we also want our system to support both functions. In addition, we require our system to allow smooth cross-referencing between EDA scripts and data stories.

\textbf{D2. Optimization for the design space.} Our design space for actionable EDA and storytelling outlines key dimensions an AI assistant can optimize for. Moreover, these dimensions subsume the challenges in EDA and storytelling: optimizing for the \semanticcolor{semantic} and \rhetoriccolor{rhetorical} dimensions jointly tackles \textbf{C1} through \textbf{C3}, and doing so for the \pragmaticcolor{pragmatic dimension} addresses \textbf{C4}. Nonetheless, to effectively bring this theoretical framework into practice, our tool needs to adopt effective strategies to operationalize the design space.

\textbf{D3. Steerability.} Our interviews revealed analysts' need for control over the AI assistant’s behavior. For instance, analysts preferred using the AI as an executor when they had clear analysis plans but desired more proactive, agentic involvement from the AI when they were uncertain or lacked direction. Therefore, we aim to provide a steerable system, one that can accurately interpret user intent and undertake the appropriate level of agency. 

\textbf{D4. Explainability.} While participants were impressed by the generative capabilities of LLMs, most expressed reservations about their lack of transparency. To address this, we will ensure our system offers explanations to enhance user understanding and trust in both EDA and storytelling. Additionally, we aim to provide a feature that allows users to engage in threaded conversations with the AI for clarification on its decisions and interpretations.

\textbf{D5. Reparability.} In many cases, analysts may want to repair the AI's responses. We will strive for two forms of reparability: direct manipulation and user-guided AI refinement. In direct manipulation, analysts manually adjust the AI's output. In user-guided AI refinement, analysts provide instructions, and the AI implements the changes accordingly. These mechanisms ensure flexibility and control, enabling analysts to refine AI contributions as needed.




